MILR: Mathematically Induced Layer Recovery for Plaintext Space Error Correction of CNNs

The increased use of Convolutional Neural Networks (CNN) in mission critical systems has increased the need for robust and resilient networks in the face of both naturally occurring faults as well as security attacks. The lack of robustness and resiliency can lead to unreliable inference results. Current methods that address CNN robustness require hardware modification, network modification, or network duplication. This paper proposes MILR a software based CNN error detection and error correction system that enables self-healing of the network from single and multi bit errors. The self-healing capabilities are based on mathematical relationships between the inputs,outputs, and parameters(weights) of a layers, exploiting these relationships allow the recovery of erroneous parameters (weights) throughout a layer and the network. MILR is suitable for plaintext-space error correction (PSEC) given its ability to correct whole-weight and even whole-layer errors in CNNs.

==> tables/CIFAR-10/CIFAR_acc.tex <==
\begin{scriptsize}
    \begin{table*}[htbp]
        \centering
        \caption{CIFAR-10 small network RBER accuracy }
        \label{tab:CIFAR_acc}
        \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
            \hline
            \textbf{Recovery}  & \textbf{ 1E-07}  & \textbf{5E-07}  & \textbf{1E-06}  & \textbf{5E-06}  & \textbf{1E-05}  & \textbf{5E-05}  & \textbf{1E-04}& \textbf{5E-04}\\
            \hline
            \hline
            None &  99.1\% &	81.5\% &	70.5\% &	24.2\% &	13.6\% &	12.0\% &	11.8\% &	11.7\%\\
            \hline
            ECC &   100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	97.8\% &	82.4\% &	16.9\%\\
            \hline
            MILR &  100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	98.8\% &	95.4\% &	80.2\%\\
            \hline
            ECC + MILR &   100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% \\
           \hline
        \end{tabular}
    \end{table*}
\end{scriptsize}


==> tables/CIFAR-10/CIFAR_acc_wholeword.tex <==
\begin{scriptsize}
    \begin{table*}[htbp]
        \centering
        \caption{CIFAR-10 small network whole-weight errors accuracy }
        \label{tab:CIFAR_acc_wholeword}
        \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
            \hline
            \textbf{Recovery} & \textbf{1E-07} & \textbf{5E-07} & \textbf{1E-06} & \textbf{5E-06} & \textbf{1E-05} & \textbf{5E-05} & \textbf{1E-04}& \textbf{5E-04}& \textbf{1E-03}\\
            \hline
            \hline
            None &  97.5\% &	87.8\% &	83.6\% &	49.5\% &	25.4\% &	11.8\% &	11.4\% &	11.8\% &	11.7\% \\
            \hline
            MILR &  100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	97.7\% &	92.0\% \\
            \hline
        \end{tabular}
    \end{table*}
\end{scriptsize}

==> tables/CIFAR_B/CIFAR_B_ACC.tex <==
\begin{scriptsize}
    \begin{table*}[htbp]
        \centering
        \caption{CIFAR-10 large network RBER accuracy }
        \label{tab:CIFAR_B_acc}
        \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
            \hline
            \textbf{Recovery}  & \textbf{ 1E-07}  & \textbf{5E-07}  & \textbf{1E-06}  & \textbf{5E-06}  & \textbf{1E-05}  & \textbf{5E-05}  & \textbf{1E-04}& \textbf{5E-04}\\
            \hline
            \hline
            None &  95.1\% &	78.5\% &	60.8\% &	16.3\% &	12.1\% &	12.2\% &	11.9\% & 12.0\% \\
            \hline
            ECC &   100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	99.5\% &	87.0\% & 12.1\% \\
            \hline
            MILR &  100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	99.7\% &	98.4\% & 86.1\% \\
            \hline
            ECC + MILR &   100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% & 100.0\% \\
           \hline
        \end{tabular}
    \end{table*}
\end{scriptsize}


==> tables/CIFAR_B/CIFAR_B_Whole.tex <==
\begin{scriptsize}
    \begin{table*}[htbp]
        \centering
        \caption{CIFAR-10 large network whole-weight errors accuracy }
        \label{tab:CIFAR_B_acc_wholeword}
        \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
            \hline
            \textbf{Recovery} & \textbf{1E-07} & \textbf{5E-07} & \textbf{1E-06} & \textbf{5E-06} & \textbf{1E-05} & \textbf{5E-05} & \textbf{1E-04}& \textbf{5E-04}& \textbf{1E-03}\\
            \hline
            \hline
            None &  98.8\% &	83.2\% &	73.2\% &	26.4\% &	12.7\% &	12.0\% &	11.6\% &	12.3\% &	12.0\% \\
            \hline
            MILR &  100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	99.9\% &	99.2\% &	93.2\% \\
            \hline
        \end{tabular}
    \end{table*}
\end{scriptsize}

==> tables/MNIST/MINST_Acc_wholeword.tex <==
\begin{scriptsize}
    \begin{table*}[htbp]
        \centering
        \caption{MNIST network whole-weight errors accuracy  }
        \label{tab:MNIST_acc_wholeWord}
        \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
            \hline
            \textbf{Recovery} & \textbf{1E-07} & \textbf{5E-07} & \textbf{1E-06} & \textbf{5E-06} & \textbf{1E-05} & \textbf{5E-05} & \textbf{1E-04} & \textbf{5E-04} & \textbf{1E-03} & \textbf{5E-03}\\
            \hline
            \hline
            None & 100.0\% &	97.3\% &	96.6\% &	85.1\% &	68.0\% &	26.4\% &	13.1\% &	10.7\% &	10.0\% &	10.0\% \\
            \hline
            MILR  & 100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	99.9\% &	94.6\% &	55.9\% \\
            \hline
        \end{tabular}
    \end{table*}
\end{scriptsize}

==> tables/MNIST/MNIST_ACC.tex <==
\begin{scriptsize}
    \begin{table*}[htbp]
        \centering
        \caption{MNIST network RBER accuracy }
        \label{tab:MNIST_acc}
        \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
            \hline
            \textbf{Recovery} & \textbf{1E-07} & \textbf{5E-07} & \textbf{1E-06} & \textbf{5E-06} & \textbf{1E-05} & \textbf{5E-05} & \textbf{1E-04} & \textbf{5E-04} & \textbf{1E-03}\\
            \hline
            \hline
            None & 99.1\% &	94.3\% &	85.6\% &	58.9\% &	37.8\% &	12.9\% &	12.9\% &	10.0\% &	10.1\%\\
            \hline
            ECC &   100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	99.5\% &	97.0\% &	43.5\% &	14.8\%\\
            \hline
            MILR &  100.0\% &	100.0\% &	100.0\% &	100.0\% &	98.7\% &	100.0\% &	99.0\% &	89.3\% &	73.2\%\\
            \hline
            ECC + MILR & 100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	100.0\% &	98.4\%\\
            \hline
        \end{tabular}
    \end{table*}
\end{scriptsize}
